ProgGen: Generating Named Entity Recognition Datasets Step-by-step with Self-Reflexive Large Language Models

Although Large Language Models (LLMs) exhibit remarkable adaptability across domains, these models often fall short in structured knowledge extraction tasks such as named entity recognition (NER). This paper explores an innovative, cost-efficient strategy to harness LLMs with modest NER capabilities for producing superior NER datasets. Our approach diverges from the basic class-conditional prompts by instructing LLMs to self-reflect on the specific domain, thereby generating domain-relevant attributes (such as category and emotions for movie reviews), which are utilized for creating attribute-rich training data. Furthermore, we preemptively generate entity terms and then develop NER context data around these entities, effectively bypassing the LLMs' challenges with complex structures. Our experiments across both general and niche domains reveal significant performance enhancements over conventional data generation methods while being more cost-effective than existing alternatives.

==> tex/gen-sample-prompts/sim-prompt.tex <==
% {\footnotesize
Suppose you are \tplVal{a news writer}. Please generate \tplVar{\#generate} synthetic \tplVal{sentences} from \tplVal{news stories}. Please identify all named entities occurred that belong to one of the following entity types:

\tplVal{[person, location, organization]}.

Please list such named entities with the corresponding entity types on the following line, in the order of occurrence.

If no entity is found in the generated sentence, leave the brackets empty.

Here are some example sentences and annotations for your reference. Please follow this format.\nl

% ~\par

Examples:\nl

% ~\par

\tplVal{Sentence: ``Saudi Arabia executes Pakistani man.''}

\tplVal{Named Entities: [Saudi Arabia (location)]\nl}

\tplVal{...}

% ~\par

% Sentence: ``BASEBALL-DODGERS WIN FIFTH STRAIGHT."

% Named Entities: [DODGERS (organization)]

% ~\par

% Sentence: ``With 2.5 percent gross domestic product growth expected for 1996, new job growth should slowly lower the unemployment rate over the rest of the year."

% Named Entities: []

% ~\par

% Sentence: ``A.de Silva not out 49"

% Named Entities: [A.de Silva (person)]

% ~\par

% \textbackslash n
% \texttt{---}
% \begin{verbatim}
% ---
% \end{verbatim}
\pptSep
% \hspace{0.05em}\verb|---|
% \hspace{0.04em}-{}-{}-
% }

